Noether: The More Things Change, the More Stay the Same

Symmetries have proven to be important ingredients in the analysis of neural networks. So far their use has mostly been implicit or seemingly coincidental. We undertake a systematic study of the role that symmetry plays. In particular, we clarify how symmetry interacts with the learning algorithm. The key ingredient in our study is played by Noether's celebrated theorem which, informally speaking, states that symmetry leads to conserved quantities (e.g., conservation of energy or conservation of momentum). In the realm of neural networks under gradient descent, model symmetries imply restrictions on the gradient path. E.g., we show that symmetry of activation functions leads to boundedness of weight matrices, for the specific case of linear activations it leads to balance equations of consecutive layers, data augmentation leads to gradient paths that have "momentum"-type restrictions, and time symmetry leads to a version of the Neural Tangent Kernel. Symmetry alone does not specify the optimization path, but the more symmetries are contained in the model the more restrictions are imposed on the path. Since symmetry also implies over-parametrization, this in effect implies that some part of this over-parametrization is cancelled out by the existence of the conserved quantities. Symmetry can therefore be thought of as one further important tool in understanding the performance of neural networks under gradient descent.

==> old.tex <==
\section{Potential ideas}

\subsection{Neural tangent kernel}

Somehow data augmentation fits the framework in a sense that it is a symmetry in data distribution. For instance here \href{https://arxiv.org/pdf/1911.00809.pdf}{convolutionalNTKArora.pdf} they show that CNN with a Global Average Pooling in the last layer is equivalent to data augmentation with all translations. But it looks like it goes in a funny direction: symmetry in a network architecture implies symmetry in the data distribution.


\subsection{Mean field methods}
\href{https://web.stanford.edu/~montanar/RESEARCH/FILEPAP/mean_field.pdf}{montanari-mean-field.pdf} In there he considers 2-layer neural network in the limit of infinite number of hidden neurons. Potential invariances and symmetries are as follows:
\begin{itemize}
    \item Symmetry of data $\xrightarrow{}$ Symmetry/invariance of distribution on weights. For example if data distribution is rotational invariant then weight distribution is rotational invariant,
    \item Naturally factoring out permutation symmetry
\end{itemize}

\subsection{Convolutional networks}

Maybe there is something here... But look at NTK section.

\subsection{Homogeneity of activation function}

Somehow the homogeneity of the activation function (that is for $p$ we say $\sigma$ is $p$ - homogenous if for all $\lambda > 0$ we have $\sigma(\lambda x) =\lambda^p \sigma(x)$) seems to be imprtant for some convergance results. For instance in \href{https://arxiv.org/pdf/1805.09545.pdf}{bach-leizac.pdf} they say: 

"The functions $\phi$ and $V$ obtained through the lifting share the property of being positively 1-homogeneous in the variable $w$. This property is central for our global convergence results (but is not needed throughout Section 2)."

This is a property that we use in Sections~\ref{sec:twolayer} and \ref{sec:canonicalform} to get a symmetry.

\section{Neural Tangent Kernel}

\subsection{Standard framework}
For a training set $\{(x_i,y_i)\}_{i=1}^n$ and parameters $\w$ we define the training loss as $\ell(\w) := \frac{1}{2} \sum_{i=1}^n (g(\w;x_i) - y_i)^2$. $g : \R^d \xrightarrow{} \R$ is our network parametrized by $\textbf{w}$. In the standard NTK we have the following dynamic:
$$
\frac{d \textbf{w}(t)}{d t} = - \nabla \ell(\textbf{w}(t)) = - \sum_{i=1}^n (g(\textbf{w}(t), x_i) - y_i) \cdot \frac{\partial f_{\w(t)}(x_i)}{\partial \textbf{w}}
$$
Then they look how the prediction of $g$ on a given training example changes with respect to time.
\begin{align*}
\frac{d f_{\w(t)}(x_i)}{dt}
&= \left\langle \frac{\partial f_{\w(t)}(x_i)}{\partial \textbf{w}} , \frac{d \textbf{w}(t)}{dt} \right\rangle \\
&= -\sum_{j=1}^n (g(\textbf{w}(t), x_j) - y_j) \cdot \left\langle \frac{\partial f_{\w(t)}(x_i)}{\partial \textbf{w}}, \frac{\partial f_{\w(t)}(x_j)}{\partial \textbf{w}} \right\rangle
\end{align*}
Now if you denote $u(t) := (g(\textbf{w}(t),x_1), g(\textbf{w}(t),x_2), \dots, g(\textbf{w}(t),x_n))^T$. Then using the above you can succinctly write
\begin{equation}\label{eq:standardNTK}
\frac{d u(t)}{dt} = - H(t) (u(t) - y) \text{,}
\end{equation}
where we set 
\begin{equation}
H_{i,j}(t) :=  \left\langle \frac{\partial f_{\w(t)}(x_i)}{\partial \textbf{w}}, \frac{\partial f_{\w(t)}(x_j)}{\partial \textbf{w}} \right\rangle \text{.}
\end{equation}
Then in the NTK (when width goes to infinity) they say that $H$ is the kernel matrix and that it doesn't change much throughout training, which means $H$ is basically a constant matrix $H^*$ defined as:
\begin{equation}
H_{i,j}^* := \mathbb{E}_{\textbf{w}}\left\langle \frac{\partial f_{\w(t)}(x_i)}{\partial \textbf{w}}, \frac{\partial g(\textbf{w}(t); x_j)}{\partial \textbf{w}} \right\rangle ,    
\end{equation}
where the expectation is taken with respect to initialization scheme of $\textbf{w}$.

\subsection{Our case}
Now for us. We have a different dynamic, probably something like:
$$
\frac{d^2 \textbf{w}(t)}{d t^2} = - \nabla \ell(\textbf{w}(t)) = - \sum_{i=1}^n (g(\textbf{w}(t), x_i) - y_i) \cdot \frac{\partial g(\textbf{w}(t); x_i)}{\partial \textbf{w}}
$$
Then we cannot really analyze $\frac{d g(\textbf{w}(t); x_i)}{dt}$ as it depends on the first derivative of $\textbf{w}(t)$ but our ODE gives en evolution for the second derivative. Thus I wanted to look at:
\begin{align*}
\frac{d^2 g(\textbf{w}(t); x_i)}{dt^2}
&= \frac{d}{dt} \left( \left\langle \frac{\partial g(\textbf{w}(t); x_i)}{\partial \textbf{w}} , \frac{d \textbf{w}(t)}{dt} \right\rangle \right) \\
&= \left\langle \frac{\partial g(\textbf{w}(t); x_i)}{\partial \textbf{w}} , \frac{d^2 \textbf{w}(t)}{dt^2} \right\rangle + \left\langle \frac{\partial^2 g(\textbf{w}(t); x_i)}{\partial \textbf{w}^2} , \left(\frac{d \textbf{w}(t)}{dt} \right)^2 \right\rangle \\
&= \sum_{j=1}^n (g(\textbf{w}(t), x_j) - y_j) \cdot \left\langle \frac{\partial g(\textbf{w}(t); x_i)}{\partial \textbf{w}}, \frac{\partial g(\textbf{w}(t); x_j)}{\partial \textbf{w}} \right\rangle + \left\langle \frac{\partial^2 g(\textbf{w}(t); x_i)}{\partial \textbf{w}^2} , \left(\frac{d \textbf{w}(t)}{dt} \right)^2 \right\rangle,
\end{align*}
where $\left(\frac{d \textbf{w}(t)}{dt} \right)^2$ is element wise squaring. The RHS looks the same like in the standard case if not for the second term. That's the problematic term I was talking about.

\begin{comment}
\section{Nesterov derivation}

$
\theta'_{t} = \theta_{t} - lr \cdot \mu \cdot v_{t} \\
v_{t+1} = \mu \cdot v_{t} + g(\theta_{t} - lr \cdot \mu \cdot v_{t}) \\
\theta_{t+1} = \theta_{t} - lr \cdot v_{t+1} 
$
\begin{align*}
\theta'_{t+1} 
&= \theta_{t+1} - lr \cdot \mu \cdot v_{t+1} \\
&= \theta_{t} - lr \cdot v_{t+1} - lr \cdot \mu \cdot v_{t+1} \\
&= \theta'_{t} + lr \cdot  \mu \cdot v{t} - lr \cdot v_{t+1} - lr \textbf{} \mu \cdot v_{t+1} \\
&= \theta'_{t} - lr \cdot (v_{t+1} - \mu \cdot v_{t} + \mu \cdot v_{t+1}) \\
&= \theta'_{t} - lr \cdot (v_{t+1} - \mu \cdot v_{t} + \mu \cdot v_{t+1}) \\
&= \theta'_{t} - lr \cdot (g(\theta'_{t}) + \mu \cdot v_{t+1})
\end{align*}
\end{comment}


\section{NTK as an instance of Noether's Theorem?}
I have no idea if this leads to anything. But if we see a conserved quantity in this context ...

To keep things simple let us assume that we have a single sample. We have a distribution for the weights. This distribution would in general depend on time but the whole point is to show that it does not. We get the equation
\begin{align*}
\dot{g}(\textbf{w}(t)) & = - \underbrace{\mathbb{E}_{\textbf{w}}[ \langle \nabla g(\textbf{w}), \nabla g(\textbf{w}) \rangle]}_{H}  g(\textbf{w}(t)).
\end{align*}
I left out the $-y$ on the right. I don't think that this makes a difference. 

If we want to put this into the standard framework perhaps we should consider the equation
\begin{align*}
\ddot{g}(\textbf{w}(t)) & = - \mathbb{E}_{\textbf{w}}[ \langle \nabla g(\textbf{w}), \nabla g(\textbf{w}) \rangle]  g(\textbf{w}(t)).
\end{align*}
The first obstacle is that the equation is for $g$ but the parameters are the $\textbf{w}$. So it seems that we should rather look at 
$$
\dot{\textbf{w}}(t) = -  g(\textbf{w}(t)) \cdot \nabla  g(\textbf{w}(t))
$$
or probably more likely we should think of a distribution of $\textbf{w}$ and see how this changes
over time. And then we want to conclude that the $H$ does not change over time, i.e., is an invariance. If we had instead the equation
$$
\ddot{\textbf{w}}(t) = -  g(\textbf{w}(t)) \cdot \nabla  g(\textbf{w}(t))
$$
then the matching Lagrangian would be
\begin{align*}
\mathcal{L}(t, \textbf{w}, \dot{\textbf{w}}) = \frac12 | \dot{\textbf{w}}|^2 - g(\textbf{w})^2.
\end{align*}
The momentum would then be
\begin{align*}
  \textbf{p} = \frac{\partial \mathcal{L}}{\partial \dot{\textbf{w}}}  = \dot{\textbf{w}},
\end{align*}
and the Hamiltonian would be
\begin{align*}
  \mathcal{L} - \textbf{p} \frac{\partial \mathcal{L}}{\partial \textbf{p}}  = \frac12 | \textbf{p}|^2 - g(\textbf{w})^2 - \langle \textbf{p},   \textbf{p} \rangle = -\frac12 | \textbf{p}|^2 - g(\textbf{w})^2.
\end{align*}
Since the functional is invariant to time this Hamiltonian would stay conserved.

I changed some signs above I think they were wrong.

\appendix

\section{Old Stuff}
Let us now generalize the above observations.
\begin{lemma}[Hamiltonian Stays Conserved if $\Lag(t, \x, \xdot)=\Lag(\x, \xdot)$ ] \label{lem:hamiltonian}
Assume that $\Lag$ does not explicitly depend on $t$, i.e., $\Lag(t, \x, \xdot)=\Lag(\x, \xdot)$. In words, the Lagrangian is invariant to time translations.
Then 
\begin{align} \label{equ:hamiltonian}
H = \Lag - \langle \xdot, \frac{\partial \Lag}{\partial \xdot} \rangle
\end{align} 
is a constant along every extremal path. The quantity $H$ is called the {\em Hamiltonian}.
\end{lemma}
\begin{proof}
We have
\begin{align*}
\frac{d}{d t} H 
& = \frac{d}{d t} (\Lag - \langle \xdot, \frac{\partial \Lag}{\partial \xdot} \rangle) \\
& = 
\langle \frac{\partial \Lag}{\partial \x}, \xdot \rangle + 
\langle \frac{\partial \Lag}{\partial \xdot}, \xddot \rangle - 
\langle \xddot, \frac{\partial \Lag}{\partial \xdot} \rangle -
\langle \xdot, \frac{d}{dt} \frac{\partial \Lag}{\partial \xdot} \rangle \\
& = \langle \frac{\partial \Lag}{\partial \x}, \xdot \rangle  - 
\langle \frac{\partial}{\partial \x} \frac{\partial \Lag}{\partial \xdot}, \xdot \rangle - \langle \frac{\partial}{\partial \xdot} \frac{\partial \Lag}{\partial \xdot}, \xddot \rangle \\
& = \langle \frac{d}{d t} (\Lag - \langle \xdot, \frac{\partial \Lag}{\partial \xdot} \rangle), \xdot \rangle  \\ 
 & = \langle \vd, \xdot \rangle \\
 & = 0.
\end{align*}
\end{proof}

\section{Old scaling}
We have
\begin{align*}
\pmb{p} & = \frac{\partial {\mathcal L}}{\partial \dot{\textbf{w}}} = \dot{\textbf{w}}, \\
H & = - \mathcal{L}+ \langle \pmb{p}, \dot{\textbf{w}} \rangle = \frac{1}{2} \|\dot{\textbf{w}} \|_2^2 + f(\textbf{w})
\end{align*}
To check this note that the ELI equation reads
\begin{align*}
\frac{\partial {\mathcal L}}{\partial t} = \frac{d}{d t} [\mathcal{L}-  \langle \frac{\partial {\mathcal L}}{\partial \dot{\textbf{w}}}, \dot{\textbf{w}} \rangle]
\end{align*}
This gives rise to the equation
\begin{align*}
0 & =
\frac{d}{d t} \left[ \frac{1}{2} \|\dot{\textbf{w}} \|_2^2 - f(\textbf{w}) - \|\dot{\textbf{w}} \|_2^2 \right] \\
& = \frac{d}{d t}  \left[  -\frac{1}{2} \|\dot{\textbf{w}} \|_2^2 - f(\textbf{w})  \right] \\
& =   - 
\langle \ddot{\textbf{w}},  \dot{\textbf{w}} \rangle 
- \langle \nabla f(\textbf{w}), \dot{\textbf{w}}\rangle
\end{align*}
\begin{align*}
\langle \ddot{\textbf{w}},  \dot{\textbf{w}} \rangle 
+ \langle \nabla f(\textbf{w}), \dot{\textbf{w}} \rangle = 0.
\end{align*}
The ELII equation reads
\begin{align*}
\frac{\partial {\mathcal L}}{\partial \textbf{w}}
=  \frac{d}{d t} \frac{\partial {\mathcal L}}{\partial \dot{\textbf{w}}}.
\end{align*}
Therefore we get the equation
\begin{align*}
- \nabla f(\textbf{w}) = \frac{d}{d t} [ \dot{\textbf{w}}] = \ddot{\textbf{w}}.
\end{align*}
This is equivalent to 
\begin{align}
   \nabla f(\textbf{w}) +  \ddot{\textbf{w}} = 0.
\end{align}
Let a generator for the symmetry be: 
\begin{equation}
\pmb{\zeta} = (w_1,-w_2)^T.
\end{equation}
By Noether's theorem the invarianct quantity is 
\begin{align*}
\langle \pmb{p},  \pmb{\zeta} \rangle - H \tau = \langle \frac{\partial {\mathcal L}}{\partial \dot{\textbf{w}}}, \pmb{\zeta} \rangle = 
\dot{w}_1 w_1 - \dot{w}_2 w_2
\end{align*}



This is essentially Newton's second law of motion and the Lagrangian represents the difference between kinetic and potential energy. Then using the same symmetry \eqref{eq:symmetry} we get that the following holds:

For a function $\varphi : \R \xrightarrow{} \R$, such that $\varphi(t_1) = \varphi(t_2) = 0$, for every $\e \geq 0$ we define:
\begin{align*}
& w_1^{\e} := (1 + \e \varphi(t)) w_1 = w_1(t) + \e \varphi(t) w_1(t) \\
& w_2^{\e} := (1 - \e \varphi(t)) w_2 = w_2(t) + \e \varphi(t) w_2(t)
\end{align*}
Now we compute
\begin{align*}
&\int_{t_1}^{t_2} \mathcal{L}(t,\textbf{w}^{\e},\dot{\textbf{w}}^{\e}) \ dt \\
&=
\int_{t_1}^{t_2} \frac{1}{2} \left( (\dot{w}_1^{\e})^2 + (\dot{w}_2^{\e})^2 - 2f(w_1^{\e},w_2^{\e}) \right) \ dt \\
&= \int_{t_1}^{t_2} \frac{1}{2} \left( ((1 +\e \varphi)\dot{w}_1 + \e \dot{\varphi} w_1)^2 + ((1 -\e \varphi)\dot{w}_2 - \e \dot{\varphi} w_2)^2  - 2f(w_1,w_2) \right) \ dt  \\
&= \int_{t_1}^{t_2} \frac{1}{2} \left( (1 +2\e \varphi)\dot{w}_1^2 + 2 \dot{w}_1 \e \dot{\varphi} w_1 + (1 - 2 \e \varphi)\dot{w}_2^2 - 2 \dot{w}_2 \e \dot{\varphi} w_2  - 2f(w_1,w_2) \right) + O(\e^2) \ dt \\
&= \int_{t_1}^{t_2} \frac{1}{2} \left( \dot{w}_1^2 + \dot{w}_2^2 - 2f(w_1,w_2) + 2\e\varphi(\dot{w}_1^2 - \dot{w}_2^2) +2\e\dot{\varphi}(\dot{w}_1 w_1 - \dot{w}_2 w_2) \right) + O(\e^2) \ dt \\
&= \int_{t_1}^{t_2} \mathcal{L}(t,\textbf{w},\dot{\textbf{w}}) +  \e \left(\dot{w}_1 \frac{d}{dt}(\varphi w_1) - \dot{w}_2 \frac{d}{dt}(\varphi w_2) \right) + O(\e^2) \ dt
\end{align*}
Using integration by parts and the fact that $\varphi(t_1) = \varphi(t_2) = 0$ we get that:
\begin{equation}
\int_{t_1}^{t_2}  \e \dot{w}_1 \frac{d}{dt}(\varphi w_1) \ dt = \int_{t_1}^{t_2}  \e \varphi w_1 \ddot{w}_1 \ dt 
\end{equation}
So we get
\begin{equation}
\int_{t_1}^{t_2}  \e \varphi \left( w_1 \ddot{w}_1 - w_2 \ddot{w}_2 \right) \ dt = 0 
\end{equation}

\begin{equation}\label{eq:easydinamicrelu}
\ddot{w}_1 w_1 - \ddot{w}_2 w_2 = 0 \text{.}    
\end{equation}

\begin{comment}
As $\textbf{w}$ is a stationary point of \eqref{eq:lagrange} we know that:
\begin{align*}
\frac{d}{d \e}\int_{t_1}^{t_2} t^3\e\dot{\varphi}(\dot{w}_1 w_1 - \dot{w}_2 w_2) \ dt = 0 \text{.}    
\end{align*}
Using integration by parts and the fact that $\varphi(t_1) = \varphi(t_2) = 0$ we get that:
\begin{equation}
\int_{t_1}^{t_2} \varphi(t) \frac{d}{dt} \left[ t^3(\dot{w}_1 w_1 - \dot{w}_2 w_2) \right] \ dt = 0 \text{.}   
\end{equation}
Using fundamental lemma of calculus of variations we get that:
\begin{equation}
\frac{d}{dt} \left[ t^3(\dot{w}_1 w_1 - \dot{w}_2 w_2) \right] = 0 \text{,}
\end{equation}
which is equivalent to:
\begin{equation}
\frac{d}{dt} \left[ t^3 \frac{d}{dt}  \left(w_1^2 - w_2^2 \right) \right] = 0 \text{.}
\end{equation}
The last equation somehow resembles Theorem 2.1 from https://arxiv.org/pdf/1806.00900.pdf, when you remove $t$ from the equation above you get that the second derivative of the difference between squared weights is zero, while in the paper it's the first derivative.
\end{comment}


\subsection{Nesterov's Accelerated Gradient Flow}

Imagine that we run the following version of an accelerated gradient descent with continuous time (considered in https://arxiv.org/abs/1603.04245) for this problem, which is a continuous version of Nesterov acceleration \href{https://www.jmlr.org/papers/volume17/15-084/15-084.pdf}{nesterovCandes.pdf}:
\begin{equation}\label{eq:accgd}
\ddot{\textbf{w}} + \frac{3}{t} \dot{\textbf{w}} + \nabla f(\textbf{w}) = 0 \text{.}
\end{equation}
Now we define a Lagrangian:
\begin{equation}\label{eq:lagrange}
\mathcal{L}(t,\textbf{w},\dot{\textbf{w}}) := t^3 \left(\frac{1}{2} \|\dot{\textbf{w}} \|_2^2 - f(\textbf{w}) \right) \text{.}    
\end{equation}
Observe that \eqref{eq:accgd} satisfies Euler-Lagrange equations for \eqref{eq:lagrange}, which means that it is a stationary point of the action functional associated with $\mathcal{L}$. To check this note that the ELI equation reads
\begin{align*}
\frac{\partial {\mathcal L}}{\partial t} = \frac{d}{d t} \left[\mathcal{L}-  \left\langle \frac{\partial {\mathcal L}}{\partial \dot{\textbf{w}}}, \dot{\textbf{w}} \right\rangle \right]
\end{align*}
This gives rise to the equation
\begin{align*}
3 t^2 \left(\frac{1}{2} \|\dot{\textbf{w}} \|_2^2 - f(\textbf{w}) \right) & =
\frac{d}{d t} \left[ t^3 \left(\frac{1}{2} \|\dot{\textbf{w}} \|_2^2 - f(\textbf{w}) \right) - t^3 \|\dot{\textbf{w}} \|_2^2 \right] \\
& = \frac{d}{d t} t^3 \left[  -\frac{1}{2} \|\dot{\textbf{w}} \|_2^2 - f(\textbf{w})  \right] \\
& =  -3 t^2 \left[  \left(\frac{1}{2} \|\dot{\textbf{w}} \|_2^2 + f(\textbf{w}) \right) \right] - 
t^3[\langle \dot{\textbf{w}},  \ddot{\textbf{w}} \rangle 
- \langle \nabla f(\textbf{w}), \dot{\textbf{w}}\rangle]
\end{align*}
\begin{align*}
  \frac{3}{t} \langle \dot{\textbf{w}}, \dot{\textbf{w}} \rangle 
+
\langle \ddot{\textbf{w}},  \dot{\textbf{w}} \rangle 
+ \langle \nabla f(\textbf{w}), \dot{\textbf{w}} \rangle = 0.
\end{align*}
This is basically the original equation but taking with an inner product with $\dot{\pmb{w}}$. Not clear why this is the same. In the derivation of the book this happens at (3.2.4) and there you use the ELII but multiplied by $\dot{\pmb{w}}$. So this is where the factor comes from. The question is why the two are equivalent.

The ELII equation reads
\begin{align*}
\frac{\partial {\mathcal L}}{\partial \textbf{w}}
=  \frac{d}{d t} \frac{\partial {\mathcal L}}{\partial \dot{\textbf{w}}}.
\end{align*}
Therefore we get the equation
\begin{align*}
- t^3 \nabla f(\textbf{w}) = \frac{d}{d t} [t^3 \dot{\textbf{w}}] = 3 t^2 \dot{\textbf{w}} + t^3 \ddot{\textbf{w}}.
\end{align*}
This is equivalent to 
\begin{align}
   \nabla f(\textbf{w}) + \frac{3}{t}  \dot{\textbf{w}} +  \ddot{\textbf{w}} = 0.
\end{align}
Let a generator for the symmetry be: 
\begin{equation}
\pmb{\zeta} = (w_1,-w_2)^T.
\end{equation}
By Noether's theorem the invarianct quantity is 
\begin{align*}
\langle \pmb{p},  \pmb{\zeta} \rangle - H \tau = \langle \frac{\partial {\mathcal L}}{\partial \dot{\textbf{w}}}, \pmb{\zeta} \rangle = 
t^3 (\dot{w}_1 w_1 - \dot{w}_2 w_2).
\end{align*}


Note that for all $c > 0,w_1,w_2 \in \R$ we have that 
\begin{equation}\label{eq:symmetry}
g_{c \cdot w_1, \frac{1}{c} \cdot w_2} \equiv g_{w_1,w_2}
\end{equation}
This follows from the fact that $\sigma$ is homogeneous. Thus we get that for every $c > 0$ a transformation $(t,w_1,w_2,\dot{w}_1,\dot{w}_2) \mapsto (t, c \cdot w_1, \frac{1}{c} \cdot w_2,\dot{w}_1,\dot{w}_2)$ is a symmetry of $\mathcal{L}$.  

Now we perform a Noether's Theorem like computation to get an invariant that is preserved by a solution to \eqref{eq:accgd}. We assume $\textbf{w}$ satisfies \eqref{eq:accgd} and we consider the following small perturbation of $\textbf{w}$ between times $t_1, t_2$. For a function $\varphi : \R \xrightarrow{} \R$, such that $\varphi(t_1) = \varphi(t_2) = 0$, for every $\e \geq 0$ we define:
\begin{align*}
& w_1^{\e} := (1 + \e \varphi(t)) w_1 \\
& w_2^{\e} := (1 - \e \varphi(t)) w_2
\end{align*}
Using \eqref{eq:symmetry} and the fact that $1-x$ is a Taylor expansion of $\frac{1}{1 + x}$ around $0$ we get that $g_{w_1^{\e},w_2^{\e}} \approx g_{w_1,w_2}$ for small values of $\e$ (THIS approximation shouldn't be problematic I think).

Now we compute
\begin{align*}
&\int_{t_1}^{t_2} \mathcal{L}(t,\textbf{w}^{\e},\dot{\textbf{w}}^{\e}) \ dt \\
&=
\int_{t_1}^{t_2} \frac{t^3}{2} \left( (\dot{w}_1^{\e})^2 + (\dot{w}_2^{\e})^2 - 2f(w_1^{\e},w_2^{\e}) \right) \ dt \\
&= \int_{t_1}^{t_2} \frac{t^3}{2} \left( ((1 +\e \varphi)\dot{w}_1 + \e \dot{\varphi} w_1)^2 + ((1 -\e \varphi)\dot{w}_2 - \e \dot{\varphi} w_2)^2  - 2f(w_1,w_2) \right) \ dt  \\
&= \int_{t_1}^{t_2} \frac{t^3}{2} \left( (1 +2\e \varphi)\dot{w}_1^2 + 2 \dot{w}_1 \e \dot{\varphi} w_1 + (1 - 2 \e \varphi)\dot{w}_2^2 - 2 \dot{w}_2 \e \dot{\varphi} w_2  - 2f(w_1,w_2) \right) + O(\e^2) \ dt \\
&= \int_{t_1}^{t_2} \frac{t^3}{2} \left( \dot{w}_1^2 + \dot{w}_2^2 - 2f(w_1,w_2) + 2\e\varphi(\dot{w}_1^2 - \dot{w}_2^2) +2\e\dot{\varphi}(\dot{w}_1 w_1 - \dot{w}_2 w_2) \right) + O(\e^2) \ dt \\
&= \int_{t_1}^{t_2} \mathcal{L}(t,\textbf{w},\dot{\textbf{w}}) +  t^3\e \left(\dot{w}_1 \frac{d}{dt}(\varphi w_1) - \dot{w}_2 \frac{d}{dt}(\varphi w_2) \right) + O(\e^2) \ dt
\end{align*}
Using integration by parts and the fact that $\varphi(t_1) = \varphi(t_2) = 0$ we get that:
\begin{equation}
\int_{t_1}^{t_2}  t^3\e \dot{w}_1 \frac{d}{dt}(\varphi w_1) \ dt = \int_{t_1}^{t_2}  \e \varphi w_1 (3t^2 \dot{w}_1 + t^3 \ddot{w}_1) \ dt 
\end{equation}
Similar equation for the above holds also for the terms $w_2$. As $\textbf{w}$ is a stationary point of \eqref{eq:lagrange} we know that:
\begin{align*}
\frac{d}{d\e} \int_{t_1}^{t_2} \mathcal{L}(t,\textbf{w}^{\e},\dot{\textbf{w}}^{\e}) \ dt \Bigg|_{\e = 0} = 0 \text{.}
\end{align*}
Combining the above we get that
\begin{equation*}
\frac{d}{d\e}\int_{t_1}^{t_2}  \e \varphi\left( w_1 (3t^2 \dot{w}_1 + t^3 \ddot{w}_1) - w_2 (3t^2 \dot{w}_2 + t^3 \ddot{w}_2)  \right) \ dt \Bigg|_{\e = 0} = 0 \text{,}     
\end{equation*}
which yields:
\begin{equation}
\int_{t_1}^{t_2}  \varphi\left( w_1 (3t^2 \dot{w}_1 + t^3 \ddot{w}_1) - w_2 (3t^2 \dot{w}_2 + t^3 \ddot{w}_2)  \right) \ dt = 0    
\end{equation}
Using fundamental lemma of calculus of variations we get that:
\begin{equation}
w_1 (3t^2 \dot{w}_1 + t^3 \ddot{w}_1) - w_2 (3t^2 \dot{w}_2 + t^3 \ddot{w}_2) = 0 \text{.}
\end{equation}

Note that (\ref{equ:basicexample}) corresponds to a set of equations, one for each component of $\textbf{w}$. We can
take the inner product of the vector on the left side of equation (\ref{equ:basicexample}) with any other vector and this inner product will have to be $0$. E.g., let us take the inner product with the "variation" $\epsilon \varphi(t) (\textbf{w}_1(t), -\textbf{w}_2(t))^T$, where we think of $\epsilon$ as a small quantity. We then get
\begin{align*}
0 & = \epsilon \varphi(t) (w_1(t), -w_2(t)) (\ddot{\textbf{w}} + \nabla f(\textbf{w})) = \epsilon \varphi (w_1\ddot{w}_1 - w_2 \ddot{w}_2) + \epsilon \varphi \langle \nabla f(\textbf{w}), (w_1,-w_2)^T \rangle .
\end{align*}
But now note that this variation keeps $f(\textbf{w})$ invariant up to linear orders in $\epsilon$. We therefore have
\begin{align*}
0 & = \epsilon \varphi(t) (w_1\ddot{w}_1 - w_2 \ddot{w}_2) + O(\epsilon^2) 
\end{align*}
for any $\varphi(t)$ as long as we consider paths $\textbf{w}(t)$ that fulfill the EL equation (\ref{equ:basicexample}). We conclude that $w_1(t) \ddot{w}_1(t) - w_2(t) \ddot{w}_2(t)=0$ along such a path.


For the gradient descent we do not have a Lagrangian but we have the equivalent of the EL equations, namely the dynamic is given by
\begin{align} \label{equ:gd}
\dot{\textbf{w}} + \nabla f(\textbf{w}) = 0.
\end{align}
As before,  if we take the vector on the left-hand side of this equation and multiply it by a variation then this inner product must be $0$. If, e.g., we take the same variation we get

\begin{align*}
0 =  \epsilon \varphi(t) (w_1(t), -w_2(t)) (\dot{\textbf{w}} + \epsilon \varphi(t) \nabla f(\textbf{w})) = \epsilon \varphi(t) (w_1\dot{w}_1 - w_2 \dot{w}_2) + \epsilon \varphi \langle \nabla f(\textbf{w}), (w_1,-w_2)^T \rangle.
\end{align*}
As before, we can use the partial symmetry to conclude that 
\begin{align*}
0 = \epsilon \varphi(t) (w_1\dot{w}_1 - w_2 \dot{w}_2) + O(\epsilon^2) = \epsilon \varphi(t) \frac{d}{d t} (w_1^2 - w_2^2) + O(\epsilon^2).
\end{align*}
Since the right-hand side is a total derivative up to higher order terms in $\epsilon$ we conclude that $w_1^2(t) - w_2^2(t)$ stays constant along any path determine by the dynamics (\ref{equ:gd}). In other words, we have found that
$w_1^2(t) - w_2^2(t)$ is a conserved quantity.

\section{Old linear}

\subsection{Newtonian Dynamics}

Now we consider ND for this network. It corresponds to the following Lagrangian:
\begin{equation}
\mathcal{L}(t,\w,\wdot) := \frac{1}{2} \|\wdot \|_2^2 - \loss(\w) \text{.}      
\end{equation}
We define now the symmetry that will be used to derive a conserved quantity. Note that for every $A \in \R^{d_i \times d_i}$ such that $\text{det}(A) \neq 0$ we have that:
\begin{equation}
(W_{i} A^{-1}) \cdot (A W_{i-1}) = W_i W_{i-1}    
\end{equation}
Now let $A \in \R^{d_i \times d_i}, \text{det}(A) \neq 0$ {\color{red} Is not even necessary as we consider later $I + \epsilon A$}. For a path $W_1(t), W_2(t)$ we will consider how the action functional changes under perturbation $W_2(t) \mapsto W_2(t) (I + \e \varphi(t) A)^{-1} = W_2^\e(t), W_1(t) \mapsto (I + \e \varphi(t) A) W_1(t) = W_1^\e(t)$. Using the Taylor expansion for the matrix inverse we will use:
$$
(I + \e \varphi(t) A)^{-1} \approx I - \e \varphi(t) A \text{.}
$$
Now we compute how the action functional changes. Norms and dot products below are Frobenius. 

\begin{align*}
&\int_{t_1}^{t_2} \mathcal{L}(t,\textbf{w}^{\e},\dot{\textbf{w}}^{\e}) \ dt \\
&=
\int_{t_1}^{t_2} \frac{1}{2} \left( \|\dot{W}_1^{\e}\|_F^2 + \|\dot{W}_2^{\e}\|_F^2 - 2f(W_1^{\e},W_2^{\e}) \right) \ dt \\
&= \int_{t_1}^{t_2} \frac{1}{2} \left( \|\dot{W}_1 +\e \varphi A \dot{W}_1 + \e \dot{\varphi} A W_1\|_F^2 + \|\dot{W}_2 -\e \varphi \dot{W}_2 A - \e \dot{\varphi} W_2 A \|_F^2  - 2f(W_1,W_2) \right) \ dt  \\
&= \int_{t_1}^{t_2} \frac{1}{2} ( \|\dot{W}_1\|_F^2 + \e \varphi \langle \dot{W}_1, A \dot{W}_1 \rangle_F + \e\dot{\varphi} \langle \dot{W}_1,  A W_1 \rangle_F + \e\varphi \langle A \dot{W}_1, \dot{W}_1 \rangle_F + \e \dot{\varphi} \langle A W_1,  \dot{W}_1 \rangle_F  \\
&+ \|\dot{W}_2\|_F^2 - \e \varphi \langle \dot{W}_2, \dot{W}_2 A \rangle_F - \e \dot{\varphi} \langle \dot{W}_2, W_2 A \rangle_F - \e \varphi \langle \dot{W}_2 A, \dot{W}_2 \rangle_F - \e \dot{\varphi} \langle W_2 A,  \dot{W}_2 \rangle_F 
- 2f(W_1,W_2) ) + O(\e^2) \ dt \\
&= \int_{t_1}^{t_2} \mathcal{L}(t,\textbf{w},\dot{\textbf{w}}) + \e \langle \dot{W}_1, \varphi A \dot{W}_1 + \dot{\varphi} A W_1 \rangle_F - \e \langle \dot{W}_2, \varphi \dot{W}_2 A + \dot{\varphi} W_2 A \rangle_F + O(\e^2) \ dt \\
&= \int_{t_1}^{t_2} \mathcal{L}(t,\textbf{w},\dot{\textbf{w}}) + \e \left\langle \dot{W}_1, \frac{d}{dt}( \varphi A W_1 ) \right\rangle_F - \e \left\langle \dot{W}_2, \frac{d}{dt}( \varphi W_2 A) \right\rangle_F + O(\e^2) \ dt
\end{align*}
Thus by integrating by parts we get that for every extremal path we must have
$$
\left\langle \ddot{W}_1, A W_1 \right\rangle - \left\langle \ddot{W}_2, W_2 A  \right\rangle = 0.$$
The above can be written in terms of the trace,
$$
\text{tr}( \ddot{W}_1^T A W_1 ) - \text{tr}( \ddot{W}_2^T W_2 A ) = 0. 
$$
Using the cyclic property of the trace this is equivalent to
$$
\text{tr}( (W_1 \ddot{W}_1^T- \ddot{W}_2^T W_2) A ) = 0.
$$
As the above holds for every invertible matrix $A$ it follows that
\begin{equation}
W_1 \ddot{W}_1^T  - \ddot{W}_2^T W_2 = 0.
\end{equation}
%Using the fact that $\text{tr}( \ddot{W}_1^T  A %W_1)=\text{tr}( (\ddot{W}_1^T  A W_1)^T)= \text{tr}( %({W}_1^T  A^T  \ddot{W}_1) = \text{tr}( \ddot{W}_1 W_1^T %A^T )$, where in the last equality we have used that %cyclic shifts do not change the trace,
%$$
%\text{tr}( \ddot{W}_1 W_1^T A^T ) - \text{tr}( %\ddot{W}_2^T W_2 A ) = 0.    
%$$
%As the above holds for every invertible matrix then %somehow this should follow
%\begin{equation}
%\ddot{W}_1 W_1^T - \ddot{W}_2^T W_2 = 0 
%\end{equation}
Looks like a perfect "generalization" of \eqref{eq:easydinamicrelu} 

\begin{lemma}
Let $X$ be an $n \times n$ matrix. Then if 
\begin{align*}
    \text{tr} (X A) = 0,
\end{align*}
for every $n \times n$ invertible matrix $A$ it follows that $X = 0$.
\end{lemma}
\begin{proof}
Using the SVD decomposition we can write $X$ as $X = U D V^T$, where $U$ and $V$ are $n \times n$ unitary matrices and $D$ is diagonal. Hence
\begin{align}
0 = \text{tr}(X A) = 
\text{tr}(U D V^T A U U^T) = \text{tr}(U D B U^T) = \text{tr}(D B),
\end{align}
where $B = V^T A U$ is any invertible matrix. In particular, picking $B$ to be $D^\dagger$ we get that:
\begin{align*}
\sum_{i=1}^{n} |d_{i,i}|^2 = 0,
\end{align*}
which means that $D$ is the zero matrix.
\end{proof}

\subsection{Nesterov's Accelerated Gradient Flow}

\subsection{Gradient Flow}

\section{NTK}

....Maybe something along these lines would work for a proof: if there exists $i$ such that $|\dot{w}_i| = \Theta(1)$ (that is much bigger velocity than the expected $1/\sqrt{m}$) then the weights "connected" to $w_i$ would typically have velocities of $\Theta(1/\sqrt{m})$ but there is $m$ of them so summing them up would contradict the constantness of the Hamiltonian. These energy arguments somehow magically give properties of no-vanishing and no-exploding gradients Hmmm ....

\subsection{Nesterov's Accelerated Gradient Flow}

For Nesterov dynamic:
$$\ddot{\textbf{w}} + \frac{3}{t} \dot{\textbf{w}} + \nabla f(\textbf{w}) = 0$$
I think if you do a similar derivation to \eqref{eq:derivation} the corresponding ODE you will get for $u$ is as follows:
$$ \ddot{u} = - E E^T (u-y) - \frac{3}{t} E \dot{\textbf{w}} \text{.} $$
where $E \in \R^{n \times m}$, where the $i$-th row is equal $\frac{\partial g(\textbf{w}(t); x_i)}{\partial \textbf{w}}$. $E E^T$ will become exactly $H$ from the previous case as the gradients don't change during training. 

Hmmm ... but the Hamiltonian in this case is something like $t^3 (\frac{1}{2}\|\dot{\textbf{w}}\|^2 + f(\textbf{w}))$, which would mean that for small $t$ $\|\dot{\textbf{w}}\|$ is huge ... but it looks like a technical problem

%And it should be even easier to prove as the constant Hamiltonian will give that:
%$$\mathbb{E}_{i \sim \{1,2\dots,m\}}|w_i(t) - w_i(0)| \leq O \left(\frac{1}{\sqrt{m} \cdot t^3} \right) \text{.}
%$$
The equation doesn't look so nice because there is an expression in $\dot{\textbf{w}}$, which makes it hard to analyze but if you really look at what are the elements of $E \dot{\textbf{w}} $ you see that:
$$
(E \dot{\textbf{w}} )_i = \left\langle \frac{\partial g(\textbf{w}(t); x_i)}{\partial \textbf{w}}, \dot{\textbf{w}} \right\rangle = \frac{d}{dt} \left( g(\textbf{w}(t); x_i) \right) \ \ :)
$$
so in the end you will get:
$$
\ddot{u} = - H(u - y) - \frac{3}{t} \dot{u},
$$
which is exactly kernel ridge regression dynamic when you use Nesterov acceleration to optimize $L(\alpha)$. So it looks like whatever optimization algorithm you use you get, in the infinite width limit for ReLu networks, that it's equivalent to kernel regression with the same learning algorithm.

\section{NAGF}

For NAGF we get the following implications. Inspired by the previous cases we try to analyze the evolution of a difference between Frobenius norms.

Let $\alpha > 0$ and compute:
\begin{align*}
&\frac{d^2}{dt^2} \left(t^{\alpha} \left[ \frac12\|W^{(h)}\|_F^2 - \frac12 \|W^{(h+1)}\|_F^2 \right] \right) \\
&= t^{\alpha} \left[ \|\dot{W}^{(h)} \|_F^2 - \|\dot{W}^{(h+1)} \|_F^2  \right] +  t^{\alpha} \left[ \langle \ddot{W}^{(h)} , W^{(h)} \rangle - \langle \ddot{W}^{(h+1)} , W^{(h+1)} \rangle \right] \\ 
&+ 2\alpha t^{\alpha-1} \left[ \langle W^{(h)}, \dot{W}^{(h)} \rangle - \langle W^{(h+1)}, \dot{W}^{(h+1)} \rangle \right] + \alpha(\alpha-1) t^{\alpha - 2} \left[ \frac12\|W^{(h)}\|_F^2 - \frac12 \|W^{(h+1)}\|_F^2 \right]
\end{align*}
Using \eqref{eq:1homogNAGFconserved} one can simplify the above to
$$
t^{\alpha} \left[ \|\dot{W}^{(h)} \|_F^2 - \|\dot{W}^{(h+1)} \|_F^2  \right]
+ \left(2\alpha - 3 \right) t^{\alpha-1} \left[ \langle W^{(h)}, \dot{W}^{(h)} \rangle - \langle W^{(h+1)}, \dot{W}^{(h+1)} \rangle \right] + \alpha(\alpha-1) t^{\alpha - 2} \left[ \frac12\|W^{(h)}\|_F^2 - \frac12 \|W^{(h+1)}\|_F^2 \right].
$$
Observing that the second summand can be written as a total derivative and denoting $g(t) := \frac12\|W^{(h)}\|_F^2 - \frac12 \|W^{(h+1)}\|_F^2$ we get
\begin{equation}\label{eq:secondderivativeNAGF}
\frac{d^2}{dt^2} \left(t^\alpha g(t) \right) = t^{\alpha} \left[ \|\dot{W}^{(h)} \|_F^2 - \|\dot{W}^{(h+1)} \|_F^2  \right]
+ \left(2\alpha - 3 \right) t^{\alpha-1} \dot{g}(t) + \alpha(\alpha-1) t^{\alpha - 2} g(t) .
\end{equation}

Inspired by the derivation for the ND we would like to bound  $\|\dot{W}^{(h)} \|_F^2 - \|\dot{W}^{(h+1)} \|_F^2$ in terms of kinetic energy. We couldn't find a conserved quantity that corresponds in spirit to the conservation of energy for the Newtonian Dynamic. We are however able to derive a \comm{GG}{I made a mistake before. It's not that simple :( If $\loss$ is bounded away from $0$ this quantity is obviously gonna grow to infinity for $t \rightarrow \infty$} \textit{semi-conserved quantity}, that is a quantity that only decreases in time. For $\beta > 0$ we will look at quantities of the form $t^\beta \left(\frac12 \|\wdot\|^2 + \loss(\w) \right)$. Computing the time derivative we see
%If you just compute
%$$
%\frac{d}{dt} \left[ t^6(\frac12 \|\wdot\|^2 + \loss(\w)) \right] = 6t^5 \loss(w).
%$$
%which clearly is positive. But generalizing you get:
\begin{align*}
&\frac{d}{dt} \left[ t^\beta \left(\frac12 \|\wdot\|^2 + \loss(\w) \right) \right] \\
&= t^\beta \left( \langle \wdot, \wddot \rangle + \langle \nabla \loss(\w), \wdot \rangle \right) + \beta t^{\beta-1} \left(\frac12 \|\wdot\|^2 + \loss(\w) \right) \\
&=t^{\beta - 1} \left [ \left(\frac{\beta}{2} - 3\right) \langle \wdot, \wdot \rangle + \beta \loss(\w) \right] && \text{Applying }\eqref{eq:NAGFdynamic}.
\end{align*}
{\color{red} INCORRECT Observe that if we set $\beta = 5$ we get that as long as $\loss(w) < 1/10$ the expression on the right hand side is negative, which means that $t^5 \left(\frac12 \|\wdot\|^2 + \loss(\w) \right)$ is decreasing. Similar result will hold as long as $\beta < 6$. From now on we will assume that $\loss(\w) < 1/10$.

As in the ND case we can bound the problematic term from \eqref{eq:secondderivativeNAGF} by $\|\wdot\|^2$. For $\alpha = 3$, using \eqref{eq:secondderivativeNAGF} we can write
\begin{align*}
\frac{d^2}{dt^2} \left(t^3 g(t) \right) 
&= \frac{1}{t^2} \left( t^{5} \left[ \frac12 \|\dot{W}^{(h)} \|_F^2 - \frac12 \|\dot{W}^{(h+1)} \|_F^2  \right] \right)
+ 3 t^{2} \dot{g}(t) + 6 t g(t) \\
&\leq \frac{1}{t^2} \left( t^{5} \left[ \frac12 \|\wdot\|^2 + \loss(\w)  \right] \right)
+ 3 t^{2} \dot{g}(t) + 6 t g(t) && \loss \geq 0 \\
&\leq  \frac{1}{t^2} \left( \epsilon^{5} \left[ \frac12 \|\wdot(0)\|^2 + \loss(\w(0))  \right] \right)
+ 3 t^{2} \dot{g}(t) + 6 t g(t) && \text{As } t^5 \left(\frac12 \|\wdot\|^2 + \loss(\w) \right) \text{ is decreasing}
\end{align*}
\comm{GG}{I'm not sure how to deal with it formally. Basiically how to evaluate this semi-conserved quantity at $0$} Thus $g(t)$ is upper bounded by a function $y(t)$ satisfying
$$
\frac{d^2}{dt^2} \left(t^3 y(t) \right) = \frac{c}{t^2} + 3t^2 \dot{y}(t) + 6t y(t).
$$
\comm{GG}{Where the $c$ is the semi-conserved quantity at $0$ or at a small time ...} Solutions to this equations are
$$
y(t) = \frac{k_1}{t^2} + k_2 + \frac{c}{3t^3}.
$$
Using the fact that $g(t) \leq y(t)$ we finally get
$$
g(t) = \frac12\|W^{(h)}(t)\|_F^2 - \frac12 \|W^{(h+1)}(t)\|_F^2 \leq \frac{k_1}{t^2} + k_2 + \frac{c}{3t^3}.
$$
This means that
$$
\lim_{t \rightarrow \infty } \frac12\|W^{(h)}(t)\|_F^2 - \frac12 \|W^{(h+1)}(t)\|_F^2 = k_2.
$$
Not sure how to think about $k_2$ but at least we see the differences converge to a constant not like in the ND case where the second derivative was bounded by $\loss(\w(0))$.
}
